On the Reliability and Explainability of Language Models for Program Generation

Recent studies have adopted pre-trained language models, such as CodeT5 and CodeGPT, for automated program generation tasks like code generation, repair, and translation. Numerous language model-based approaches have been proposed and evaluated on various benchmark datasets, demonstrating promising performance. However, there is still uncertainty about the reliability of these models, particularly their realistic ability to consistently transform code sequences. This raises the question: are these techniques sufficiently trustworthy for automated program generation? Consequently, Further research is needed to understand model logic and assess reliability and explainability. To bridge these research gaps, we conduct a thorough empirical study of eight popular language models on five representative datasets to determine the capabilities and limitations of automated program generation approaches. We further employ advanced explainable AI approaches to highlight the tokens that significantly contribute to the code transformation. We discover that state-of-the-art approaches suffer from inappropriate performance evaluation stemming from severe data duplication, causing over-optimistic results. Our explainability analysis reveals that, in various experimental scenarios, language models can recognize code grammar and structural information, but they exhibit limited robustness to changes in input sequences. Overall, more rigorous evaluation approaches and benchmarks are critical to enhance the reliability and explainability of automated program generation moving forward. Our findings provide important guidelines for this goal.

==> sections/copytext.tex <==

\section{Result}
To answer the aforementioned RQs, we perform an extensive analysis of the generated code sequences and their explanation results, respectively.
Below, we present the results with respect to our three research questions.

\input{tables/tab1_performance_overview.tex}

\subsection{(RQ1) How do language models perform on program generation tasks?}
\smallsection{Approach}
To better understand how well the pre-trained language models are in automated program generation, we extensively study and compare their performance on the studied datasets.
We follow the same training/validation/testing data splits and fine-tuning procedure for each dataset introduced in Section~\ref{sec:dataset}.
We employed a beam search setting of one for our evaluations. 
Then, we calculated the accuracy (i.e., the exact match rate) for each model. Table~\ref{tab:tab1_performance_compare} presents a detailed summary of the accuracy achieved by eight different language models across these datasets.



\smallsection{Result}
We observe from Table~\ref{tab:tab1_performance_compare} several key findings on language model performance on program generation tasks.
First, we find that language models exclusively pre-trained on natural language corpora, such as T5, demonstrate limited effectiveness on programming tasks compared to models pre-trained on code data.
For example, T5 achieves just 6.42\% and 2.75\% accuracy on \textit{Android\_S} and \textit{Android\_M} respectively, highlighting the importance of domain-specific pre-training in improving performance on automated program generation
Additionally, we observe that model architecture plays a significant role in performance. 
Decoder-only (CodeGPT) and encoder-only (CodeBERT) models exhibit inferior results across multiple datasets compared to encoder-decoder architectures like CodeT5. 
Furthermore, we observe that models such as CodeT5, CodeReviewer, and CodeT5+ consistently outperform others across various benchmarks. 
For example, on the code+comment-to-code \textit{CodeReview} dataset, CodeReviewer obtains state-of-the-art performance with 30.43\% accuracy. Similarly, it leads text-to-code performance on the 
\textit{CONCODE} dataset with 22.65\% accuracy.
In other code-to-code scenarios, like the Tufano~\ea benchmarks, CodeT5+ performs better on multiple datasets, e.g., achieving 11.36\% accuracy on \textit{Android\_M}.
These findings are in alignment with previous studies, confirming the superiority of these models in program generation tasks~\cite{li2022codereviewer, hong2022commentfinder, wang2023codet5+}.


However, a critical observation is that the overall accuracy levels across all models are relatively low, especially in more complex tasks, which raises significant concerns about their reliability in real-world settings. 
When comparing dataset sizes, it is evident that all models perform better on small-sized datasets than on medium-sized ones. 
For example, CodeT5+'s accuracy fluctuates markedly from 18.44\% on the small \textit{B2F\_S} dataset down to just 7.84\% on the medium \textit{B2F\_M} dataset.
Additionally, the performance gap across different datasets is striking, as seen with CodeT5+, which achieves a high of 70.6\% on \textit{C\#2Java} but decreases to a mere 7.27\% on \textit{Google\_M}. 
Such fluctuations and inconsistency in results pose substantial challenges in understanding why models perform so well or poorly on specific datasets.
Understanding the reasons is crucial for future research, particularly for improving the reliability and practical application of automated program generation.

\find{\textbf{Finding 1:}
Pre-trained encoder-decoder-based models like CodeReviewer and CodeT5+ show superior performance compared to other models across diverse datasets. 
However, their inconsistent accuracy and significant variability across different tasks and datasets raise concerns about their reliability, emphasizing the need for a deeper understanding of factors affecting model behavior in downstream tasks.  
}



% \smallsection{Result}
% We can observe that, for most datasets, the pre-trained code generation models (e.g., CodeT5) significantly outperform the standard Transformer model (i.e., T5).
% Note that the performance of T5 and CodeTrans is obviously inferior to the other pre-trained code generation models.
% For example, on the dataset $Android_{S}$, T5 only obtained an accuracy of 6.38\, while the performance of CodeT5 and CodeReviewer is two times higher (i.e., 13.8\% and 14.72\% respectively). 
% This result shows that T5 cannot achieve good performance on automated code generation tasks, which is consistent with prior work~\cite{zeng2022extensive, li2022codereviewer}.
% A possible explanation is that the T5 model is not pre-trained on large-scale code corpora but only pre-trained on a large natural language corpus.
% Interestingly, CodeTrans achieves a poor performance which is even worse than T5 on the following datasets ($Google$, $Ovirt$, $TOSEM'19$, $FSE'22$ and $NIPS'21$). 
% This result could be attributed to the fact that CodeTrans is designed for the \textit{code-to-commit} task and is only pre-trained on a small scale of Java corpus while CodeT5, CoText, and CodeReviewer are pre-trained on multiple programming languages.
% In all four datasets, CodeT5 and Codereviewer perform much better than the other three NMT models. 
% These observations are also consistent with prior works~\cite{li2022codereviewer, hong2022commentfinder}.

% Interestingly, there are significant performance fluctuations on different datasets by the same code generation model.
% Note that on the datasets \textit{ICSE'19} and \textit{TOSEM'19}, the code models achieve better performance on small tokens than on medium tokens.
% Specifically, Table~\ref{tab:tab1_performance_compare} shows that T5 achieves an accuracy of 6.38\% for $Android_{S}$, which is 138\% ($\frac{6.38-2.68}{2.68}$) higher than the accuracy for $Android_{M}$.
% These results are in line with previous studies~\cite{tufano2019empirical, tufano2019learning}, which suggest that code generation models present difficulties in learning and generating long code sequences. 
% In addition, it is apparent from Table~\ref{tab:tab1_performance_compare} that the performance of code generation models fluctuates significantly across different datasets.
% In particular, CodeT5 achieves a superior performance on the dataset \textit{NIPS'21} $c\#2java$ (accuracy=69.30\%) while obtaining only 4.82\% accuracy on $Google_{M}$.
% In the code refinement scenarios, code generation models achieved the highest accuracy on $FSE'22$.
% For instance, CodeReviewer achieves an accuracy of 29.51\% for the $FSE'22$, compared with the accuracy of up to 25.49\% for $ICSE'19$ and the accuracy of up to 18.18\% for $TOSEM'19$.
% These differences can be explained in part by the fact that pre-trained models can perform better on code refinement tasks \textit{code\&comment-to-code} (i.e., $FSE'22$) compared with the \textit{code-to-code} tasks (i.e., $ICSE'19$ and $TOSEM'19$).


% We find that most of our results are consistent with the original results.
% For instance, the accuracy is 29.51\% in our study is closely similar to  30.32\% that is achieved by Zeng~\ea~for CodeReviewer under the \textit{FSE'22} dataset.
% Meanwhile, our standard transformer (T5) achieves an accuracy of 16.89\%, which is similar to 16.45\% that is achieved by Thongtanunam~\ea~\cite{Patanamon2022AutoTransform} for the $Ovirt_{S}$ dataset.
% The small performance deviations between our experimental results and the original results are acceptable due to the model randomness~\cite{zeng2022extensive}.  
% Overall, this finding demonstrates that we are able to replicate the performance of previous studies targeting NMT-based automated code generation.


% In summary, these results draw the following three implications:
% (1) The promising performance of code generation models observed in prior works can overall be replicated; and 
% (2) Different models achieve different accuracy for different datasets.







\subsection{(RQ2) How reliable are automated program generation approaches?}
Reliability and trustworthiness are critically important in automated program generation, especially within the evolving landscape of software engineering~\cite{lo2023trustworthy}.
Our preliminary investigation (RQ1) revealed a large disparity in the performance of language models: while some models demonstrated exceptionally high performance on certain datasets yet exhibited markedly lower effectiveness on others. 
This considerable fluctuation raises concerns about the potential overestimation or underestimation of their capabilities due to experimental biases.
Considering the potential for both overconfidence and undue skepticism resulting from these inaccuracies, it is crucial to measure these tools' effectiveness accurately, ensuring their proper application and deployment in software engineering practices.
In response to these issues, we undertake an in-depth analysis to uncover potential sources of unrealistic performance evaluation.
Our analysis is structured along three different aspects:
\begin{itemize}
    \item \textbf{Data Similarity between Training and Testing Sets.} 
    We investigate how similarities or duplications within training and testing datasets might inflate the perceived performance of language models. 
    Such overlaps may create an illusion of high accuracy, masking the true capabilities of these models in novel or diverse scenarios.
    \item \textbf{Data Duplication across Testing Sets.} 
    We investigate the presence of duplicate examples within testing datasets.
    Duplication within these sets can lead to a misleading evaluation.
    \item \textbf{Output-Input Similarity Analysis.} Finally, we examine the correlation between the outputs generated by the models and their inputs. In automated program generation, the expectation is for models to update or refine input code creatively and accurately. However, when outputs are the same as inputs, it raises questions about the true generative capacity of the models.
\end{itemize}

In our analysis, we utilize the BLEU score, specifically the \textit{BLEU-4} variant, to systematically evaluate the similarity within the studied datasets.
\textit{BLEU-4}, which assesses the co-occurrence of 4-gram sequences, is widely used in prior research~\cite {zeng2022extensive, Patanamon2022AutoTransform, hou2023large}.
A \textit{BLEU-4} score of 0 corresponds to no similarity, indicating completely unique content, while a score of 1 reflects total duplication or exact replication. 
By applying this metric, we can discern the extent to which our datasets contain unique or duplicative examples, thereby providing an empirical basis for evaluating the potential impact of data similarity on evaluation performance.


\subsubsection{Data Similarity between Training and Testing Sets}
In automated program generation, the robustness of language model evaluations is crucial. 
A key threat to this robustness is 'data snooping', a pitfall where models, due to improper data handling, gain inadvertent access to testing information during training~\cite{she2023pitfalls}. 
Such exposure can lead to exaggerated performance metrics as models may simply recall information rather than apply learned patterns to new data. 
To prevent this and ensure genuine model generalization, it is essential to assess the overlap between training and testing datasets.

\smallsection{Approach}
To determine the similarity score for a test instance $t$, we compare its source sequence against each instance in the training set $T = \{t_1, t_2, ..., t_n\}$. The similarity score, $S(t)$, is the maximum BLEU-4 score obtained from these comparisons:

\begin{equation}
S(t) = \max_{t_i \in T} \text{BLEU-4}(t, t_i)
\end{equation}

Additionally, we keep track of the index $i$ that yields this maximum score, which can be defined as:

\begin{equation}
i_{\text{max}}(t) = \argmax_{t_i \in T} \text{BLEU-4}(t, t_i)
\end{equation}

This iterative process is performed for each test instance $t$, allowing us to quantify the extent of data overlap and identify the potential duplication within the datasets.




\begin{figure}[t]
  \centering
  \includegraphics[width=1.02\textwidth]{figs/fig_train_test_duplicates.pdf}
  \caption{Distribution of Test-Training Data Similarity and Model Performance across Dataset
  }
  \label{fig:fig_train_test_duplicates}
\end{figure}



\smallsection{Result}
Figure~\ref{fig:fig_train_test_duplicates} and Table~\ref{tab:tab2_duplication_changes_codet5} present a detailed analysis of the data similarity between training and testing datasets and its influence on model performance.
Figure~\ref{fig:fig_train_test_duplicates} presents the distribution of test data similarity to training data across various datasets and corresponding recalculations of model performance for each similarity range.
Furthermore, we have recorded the average similarity score of the output sequences for each test instance with their most similar training instances, as shown in Figure~\ref{fig:fig_train_test_duplicates}.


Our analysis uncovers a wide variation in the similarity scores across an array of datasets, with the notable exception of the \textit{CodeReview} dataset, which stands out due to its lack of highly similar instances.
However, datasets such as \textit{Ovirt\_M} show that a majority, exceeding 60\%, of test data source sequences have a similarity score above 0.8, highlighting a considerable overlap with the training data. 
In particular, from \textit{Tufano et al.}, comprising \textit{Android\_S}, \textit{Android\_M}, \textit{Google\_S}, \textit{Google\_M}, \textit{Ovirt\_S}, and \textit{Ovirt\_M}, along with the \textit{CodeTrans-Dataset} datasets \textit{Java2C\#} and \textit{C\#2Java}, we find a significant presence of test samples that are duplicates of the training set (i.e, similarity score = 1).
For example, in all \textit{Tufano et al.} datasets, more than 20\% of the test samples are identical to those in the training set.
These findings suggest the presence of data duplication within the datasets, raising important questions about the possibility of data snooping that could distort the evaluation of model performance.

In Figure~\ref{fig:fig_train_test_duplicates}, we observe an increase in the similarity of target sequences corresponding to an increase in source sequence similarity, up until the source are completely identical ($S(t)=1$). 
Taking the \textit{Android\_S} dataset as an example, the average similarity for target sequences climbs from 0.1 to approximately 0.6 as the similarity of the source sequences increases. 
This indicates that target sequences are generally more aligned when the sources are more similar.
However, when the source sequences are identical ($S(t)=1$), the similarity between target sequences notably drops.
For example, in \textit{Android\_S}, the average similarity on target sequences drops from 0.6 to 0.4.
This observation may indicate a research oversight during dataset preparation, where instances with identical "source + target" pairs are usually removed, but those with identical sources or targets, when considered separately, remain unfiltered. 


Figure~\ref{fig:fig_train_test_duplicates} presents how language model accuracy improves as testing instances become more similar to the training data.
For instance, CodeT5+ show an accuracy of around 10\% for test instances with a similarity score below 0.2, which increases to nearly 25\% for instances above 0.8 in the \textit{B2F\_S} dataset., as shown in Table~\cite{}
this actually suggest that .... generazility.....of language models for ..., language models can not unseen or new test instances ... for future research, how to improve it is open challenges.
Interestingly, we observe a sharp decline in performance when the source seequncee are identical,, which aligns with the drop in output sequence similarity. 
first possible reason it the researcher when data preparation will remove the duplicates that "source + target" are identical
....



\input{tables/newtab2_duplication_of_codet5}

Table~\ref{tab:tab2_duplication_changes_codet5} contrasts the performance of code generation models before and after the removal of test instances with high BLEU-4 similarity scores.
Apart from \textit{CodeReview}, which lacks similar samples, a noticeable performance decline occurs when test samples with a BLEU score over 0.6 are removed.
In the \textit{Android\_S} dataset, for instance, the accuracy of \textit{CodeT5+} decreases from 15.2\% to 13.09\%. In some cases, the drop is even more pronounced; \textit{CodeT5+} falls from 70.6\% to 53.09\% on the \textit{C\#2Java} dataset.
This decline in accuracy reinforces the need for diverse and representative test sets to accurately gauge a model's generative capabilities.

\find{\textbf{Finding 2:}
Our findings highlight that while increased input similarity between training and testing data typically inflates performance metrics, identical inputs paired with variant targets lead to a noticeable performance drop. This suggests that models may overfit to training data, hindering their ability to generalize when presented with new but similar problems.}





\begin{figure}[t]
  \centering
  \includegraphics[width=1.02\textwidth]{figs/fig_within_test_duplicates.pdf}
  \caption{Distribution of Data Duplication within Testing Sets and Corresponding Model Performance Metrics
  }
  \label{fig:fig_train_test_duplicates}
\end{figure}


\subsubsection{Data Duplication across Testing Sets}
In the evaluation of automated program generation models, the presence of duplicated test instances can significantly skew results. Such duplications may lead to inflated performance measures if models are merely repeating learned inputs rather than generating novel code sequences.

\smallsection{Approach}
For each test instance $t$, we investigate potential duplication within the test set by comparing its source sequence with that of every other test instance. The maximum BLEU-4 score from these comparisons is recorded, along with the index of the test instance that yields this maximum score:

\begin{equation}
D(t) = \max_{\substack{t' \in \mathbf{T}_{\text{test}} \\ t' \neq t}} \text{BLEU-4}(t, t')
\end{equation}

\begin{equation}
j_{\text{max}}(t) = \argmax_{\substack{t' \in \mathbf{T}_{\text{test}} \\ t' \neq t}} \text{BLEU-4}(t, t')
\end{equation}

Here, $D(t)$ is the duplication score for the test instance $t$, and $j_{\text{max}}(t)$ is the index of another test instance $t'$ that is most similar to $t$. This process is iteratively performed for each test instance in the dataset, allowing us to pinpoint exact and near-duplicates within the test set.

\smallsection{Results}
Figure~\ref{fig:fig_train_test_duplicates} shows the distribution of similarity within the test data across various datasets. In examining these results, we find that certain datasets contain numerous instances where test samples closely replicate others within the same set.

For instance, the analysis indicates that in datasets such as \textit{Android\_S} and \textit{Android\_M} from \textit{Tufano et al.}, there is a significant percentage of test instances with a high degree of duplication. These findings are pivotal as they suggest that some datasets may be prone to over-representation of particular code patterns within the test set, which could falsely amplify a model's perceived accuracy.





\subsubsection{Output-Input Similarity Analysis.}




% \smallsection{Data Duplication}
% Prior studies~\cite{ahmed2022multilingual, shi2022evaluation} found that duplicated data across training and testing could lead to unrealistic model performance. 
% However, the prior studies only focus on code completion and code summarization tasks.
% Yet, little is known if the impact of data duplication also holds true for code generation models.
% % Therefore, we further confirm the trained models are capable of generating new code sequences rather than repeating the sequences existing in the training data. 
% To achieve this, we investigate the impact of the data duplication on the code generation models by comparing the accuracy of the models when the model is tested on a duplicated dataset (i.e., some instances are duplicated between training and testing dataset) and de-duplicated dataset (i.e., no duplicated instances between training and testing dataset).
% Then, we measure the performance difference between the two settings using accuracy and BLEU scores.



% \smallsection{Result}
% Table~\ref{tab:tab2_duplication_changes_codet5} summarizes the duplication rates of the studied datasets.
% We can observe that data duplication widely exists in the code generation datasets.
% Table~\ref{tab:tab2_duplication_changes_codet5} shows that the average duplicated rate in the studied datasets is 19.27\% and the duplication rate of dataset $BFP_{S}$ is even up to 45.36\%. 
% This finding indicates that it is necessary to explore the impacts of data duplication on code generation task
% Table~\ref{tab:tab2_duplication_changes_codet5} presents the performance changes of T5 and CodeReviewer. 
% We observed that after the data duplicates are removed, pre-trained programming language models show a decreased performance.
% Without the duplicated data, the accuracy of T5 drops upon 45\% on the dataset $Ovirt_{S}$ (i.e., from the accuracy of 16.89\% to 9.23\%).
% Similarly, the accuracy of CodeReviewer decreases from 25.49\% to 14.64\% on $Ovirt_{S}$.
% Besides that, we observe a slight decrease in BLEU scores after removing data duplication. 
% Overall, these results suggest that the data duplication across the training and testing datasets leads to the over-optimistic performance observed in prior research. 




% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.8\textwidth]{figs/fig_example_input_insensitivity.pdf}
%   \caption{An example of insensitive code generation}
%   \label{fig:fig_example_input_insensitivety}
% \end{figure}

\smallsection{Model Sensitivity}
Pre-trained code generation models are expected to understand inputs and generate new code differently from the input sequences.
However, code generation models sometimes can't understand how to generate new code sequences.
Thus, the generated code could potentially be the same as the input sequences, providing an inaccurate prediction.
Similarly, Thongtanunam~\cite{Patanamon2022AutoTransform} found that code tokens that should be changed remain unchanged, while code tokens that should remain unchanged are changed.
Figure~\ref{fig:fig_example_input_insensitivety} presents an example of the model sensitivity issue, where the code (i.e., prediction) is generated as the same as the source, which is incorrect when compared to the target (i.e., the ground-truth).
This means that the model is insensitive to learn any patterns between the input and output sequences.
To do so, we introduce a Changed Code Rate (\textit{CCR}) as a measure of the sensitivity of the code models for automated code generation.
Specifically, the Changed Code Rate is computed as the percentage of the generated code sequence that includes changes when compared to the input sequence from the total number of testing instances.
In particular, we focus on two types of Changed Code Rate, i.e., with considering special tokens (i.e., operators and separators) $CCR_\mathrm{w}$ and without considering special tokens $CCR_\mathrm{w/o}$.



\smallsection{Result}
Figure~\ref{fig:fig2_sensetive_unchanged_android_s} shows the evaluation results of the studied code generation models on the dataset $Android_{S}$.
Results show that although the $CCR_{w}$ of T5 and CoTexT is large, the $CCR_{w/o}$ is lower than 30\%, which means that T5 and CoTexT generate a large number of unchanged sequences regardless of special tokens.
In contrast, the $CCR_{w}$ and $CCR_{w/o}$ of CodeT5, CodeTrans, and CodeReviewer are quite close (e.g., 59.63\% and 58.60\% for CodeT5).
Note that the accuracy of CodeT5 and CodeReviewer is quite similar, but both the $CCR_{w}$ and $CCR_{w/o}$ of CodeReviewer are much larger than CodeT5. 
This interesting finding suggests that although CodeReviewer obtained a similar perfect prediction rate with CodeT5, the model is much more sensitive to generating new code. 
In summary, these results indicate that the existing code generation models suffer from code update insensitivity regardless of the accuracy of the models.

Table~\ref{tab:tab4_sensetive_unchanged_codereviewer} shows the evaluation results of CodeReviewer on all studied datasets.
Although Figure~\ref{fig:fig2_sensetive_unchanged_android_s} demonstrates that CodeReviewer is the most sensitive model with the largest $CCR_{w}$ and $CCR_{w/o}$ value on $Android_{S}$, it could not prove that CodeReviewer is nearly perfect.
As shown in Table~\ref{tab:tab4_sensetive_unchanged_codereviewer}, the $CCR_{w/o}$ of CodeReviewer is only 52\% on the dataset $BFP_{M}$, indicating that half of the generated sequences by CodeReviewer is unchanged.
It is apparent from this table that when CodeReviewer achieves higher accuracy on one dataset, the $CCR_{w}$ and $CCR_{w/o}$ are usually smaller.
For example, CodeReviewer has an accuracy of 66.1\% and $CCR_{w}$ of 98.3\% on $c\#2java$, while it gets a lower accuracy (i.e., 6.86\%) and smaller $CCR_{w}$ (i.e., 62.77\%) on $Google_{M}$.
These results suggest that the accurate CodeReviewer is insensitive to code generation.
Thus, our findings shed some light as an opportunity for future works to address this challenge and improve the robustness of code generation models.

\input{tables/newtab_input_output_duplicates}

\find{\textbf{Answer to RQ2:}
Code generation models can not provide an effective prediction for new code sequences with a reliable foundation.
Data duplicates between the training and testing data exaggerate the code generation performance.
Code generation models suffer from input insensitivity, producing many unchanged code sequences.
}



\subsection{(RQ3) Can we explain why automated code generation approaches can (or fail to) generate code sequences reliably?}

%\input{tables/tab8_explanation_compare.tex}

%\smallsection{Comparison of different XAI techniques}
%\yue{romve the comparison, change to argue}
We introduce SHAP approaches to explain pre-trained code generation models.
We focus on two aspects: (1) explanation analysis on the same dataset using distinct code generation models, and (2) explanation analysis on the distinct datasets using the same code generation models.
%in Section~\ref{sec:model_explain_AI_approach}.
%Although these approaches have been employed in code-based tasks, prior studies have not demonstrated which approach is the most effective~\cite{zhang2022diet, wang2021wheacha, wan2022they}.
% Firstly, we determine to evaluate which explainable approaches are the most effective for explaining automated code generation. 
% Unfortunately, there is no quantitative evaluation metric for explainable AI approaches in automated code generation.
% In this study, we measure and analyze the runtime efficiency and variability of explanations.
% Regarding the runtime efficiency, we compute the average value of memory usage and time usage to generate explanations for predictions.

% In terms of the variability of explanations, we utilize the average values of range and standard deviation values. 
% Code generation models are expected to focus more on key tokens to produce new code sequences.

% \smallsection{Result}
% Table~\ref{tab:tab_compare_exp_methods} reveals that the range and standard deviation values of explanation vectors by attention mechanism are much less than that by IG and SHAP.
% This finding indicates that the attention mechanism is not good as IG and SHAP to capture the differences in model behaviors. 
% Regarding IG and SHAP, Table~\ref{tab:tab_compare_exp_methods} presents that SHAP is more resource-efficient and runtime-efficient.
% Consequently, we use the SHAP approach to analyze and understand code generation models in this study.

% \find{\textbf{Result 4:}
% SHAP is more efficient and effective in explaining code generation models.
% }

% Therefore, we calculate the range and standard deviation values of explanation vectors.
% We propose two evaluation metrics to qualify the explanation, referring to Sensitivity On Code Changes(SOCC) and similarity. 
% An effective model is expected to comprehend the input code and locate the tokens that need to be updated.
% Then, the trained model recommends new code sequences. 
% Thus, we use SOCC to show how much the explanations focus on updated tokens.
% If the SOCC is higher, we think the XAI approach is more effective. 

% \begin{equation}
%     SOCC = avg(\frac{\sum r_{i} \cdot u_{i}}{\sum r_{i}})
% \end{equation}

% \begin{equation}
%     Similarity = \frac {\sqrt{ (a_{1}-a_{1}^{'})^{2} +...+(a_{n}-a_{n}^{'})^{2} ) } } {n}
% \end{equation}

% Where the feature importance $r_{i} = (a_{1},...,a_{n})$ and $u_{i}$ is a 1-0 vector to refer to the code changes. 



\smallsection{Explanation analysis on different code generation models}
As discussed earlier, distinct pre-trained programming language models perform differently on the same datasets.
Despite a number of studies indicating that specific-purpose pre-trained models can achieve better performance, it is still unclear what critical knowledge different pre-trained models capture. 
We hope to analyze the explanations of pre-trained models to find out why they present different performances.
To achieve that, we compare the explanation results of different pre-trained models. 
We analyze five types of tokens, including: 

\begin{itemize}
    \item \textbf{Identifiers} are unique names for variables, classes, methods, etc.
    \item \textbf{Keywords} refer to programming language-specific words with predetermined standard meanings.
    \item \textbf{Operators} are special symbols that represent some operation on data.
    \item \textbf{Separators} are special symbols used to indicate the group of code.
    \item \textbf{Literals} refer to constant values.
\end{itemize}

Also, we compare the feature importance between changed tokens and unchanged tokens.
The term "changed tokens" refers to source tokens requiring changes (e.g., remove, add, revise), whereas "unchanged tokens" do not require modifications between the source and target sequences.
Figure~\ref{fig:fig3_similarity_different_models}, Figure~\ref{fig:fig4_similarity_of_token_types_of_different_models} and Table~\ref{tab:tab6_exp_changes_unchanges_models} show the explanation results of code generation models on the dataset $Android_{S}$.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.6\textwidth]{figs/fig1_model_exps_similarity.pdf}
  \caption{Similarity with different models on $Android_{S}$. The larger the similarity value, the darker the color will be. 
  %\yue{Models have different performances, based on comparing their explanations, showing they learn different things. Some interesting like CodeReviewer is based on CodeT5, similar performance and we observe that their explanation is similar}
  }
  \label{fig:fig3_similarity_different_models}
\end{figure}

\smallsection{Result}
Figure~\ref{fig:fig3_similarity_different_models} compares the similarity of feature importance of five different code models on the same $Android_{S}$.
To measure similarities, we compute the Euclidean distance~\cite{barua2012mwmote} between two feature importance vectors generated by two models and then calculate the average score for one dataset.\yue{remember to add a math repre}
Figure~\ref{fig:fig3_similarity_different_models} shows some differences in what critical information distinct models focus on. 
For example, although CodeT5 is built on the same architecture as T5, their inference reasons are quite different, which suggests that pre-training on programming language codes changes model behaviors.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.75\textwidth]{figs/Fig3_Android_s_models_token_types.pdf}
  \caption{Average feature importance ($\bar{r}$) of token types highlighted by different code generation models on $Android_{S}$.
  }
  \label{fig:fig4_similarity_of_token_types_of_different_models}
\end{figure}


\input{tables/tab7_sensentive_models_explanation.tex}

Figure~\ref{fig:fig4_similarity_of_token_types_of_different_models} further details feature importance when code generation models transform code sequences. 
What stands out in the table is that all code generation models focus more on keywords compared with other types of tokens.
For CodeT5, the average $\bar{r}$ of keywords is 0.0147, while the value on the literals is only 0.0086, indicating that the average feature importance of keywords is 70.9\% ($\frac{0.0147-0.0086}{0.0086}$) higher than the feature importance of literals.
Similarly, the average $\bar{r}$ of keywords for T5 is much higher than that of the other four types of tokens.
This result indicates that keywords are the most important information for the models to generate new code.
Another observation is that there are some distinct differences in key token types between different models, which is consistent with Figure~\ref{fig:fig3_similarity_different_models}.
Figure~\ref{fig:fig4_similarity_of_token_types_of_different_models} presents that the average $\bar{r}$ of literals for CodeTrans is 0.0102, which is much higher than that of operators and separators (i.e., 0.0089 and 0.007 respectively).
On the contrary, literals are the least important token types for other code generation models.
These results are consistent with data obtained in Figure~\ref{fig:fig3_similarity_different_models}.

Table~\ref{tab:tab6_exp_changes_unchanges_models} shows the differences in feature importance that code generation models have between changed tokens and unchanged tokens.
Note, the average feature importance on each changed token is smaller than the average value on the unchanged token.
When comparing the ratio $\bar{r}_{change}/\bar{r}_{unchange}$, we observe that insensitive models pay less attention to changed tokens.
T5 has a very small $CCR_{w/o}$ (i.e., 21.1\%), and Table~\ref{tab:tab6_exp_changes_unchanges_models} shows that the ratio of $\bar{r}_{change}$ to $\bar{r}_{unchange}$ is only 0.7, suggesting that T5 pays much less attention to changed tokens compared with unchanged tokens.
Contrary to T5, the $CCR_{w/o}$ of CodeReviewer is larger and the ratio is higher.
The evidence thereby supports that if the code generation model can capture the update tokens of inputs, the model is usually more sensitive to generating new code sequences.



% \find{\textbf{Result 5:}
% Distinct code generation models capture different information to make a prediction. However, keywords are the most important tokens when models generate new code sequences. 
% }

\smallsection{Explanation analysis on different datasets}
Table~\ref{tab:tab1_performance_compare} depicts that there is a significant difference in model performance on the studied datasets.
In this section, we aim to analyze the explanation results on the different datasets. 
To achieve that, we use the SHAP approach to explain the state-of-the-art CodeReviewer on the four studied datasets.


\begin{figure}[t]
  \centering
  \includegraphics[width=0.75\textwidth]{figs/Fig4_Codereviewer_on_diff_token_tyopes.pdf}
  \caption{Average feature importance ($\bar{r}$) of token types highlighted by the model CodeReviewer on the studied datasets\protect\footnotemark.}  
  %\yue{Similar, but we find that when input have larger length, models are focus more on Separators, less on identifiers and keywords, -> less accurate}  
  \label{fig:fi4_token_types_exp_codereviewer}
\end{figure}

\footnotetext{Note that the dataset $FSE'22$ is excluded since it is challenging to distinguish the token types from the source code of $FSE'22$ due to the abundance of comments.}

\input{tables/tab9_sensetive_diffrent_data_codereviewer_exp.tex}

\smallsection{Result}
Figure~\ref{fig:fi4_token_types_exp_codereviewer} presents the average feature importance of token types captured by CodeReviewer.
What stands out in the table is that the average value $\bar{r}$ on the medium-size datasets is much larger than the value $\bar{r}$ on the small-size datasets.
For example, the feature importance $\bar{r}$ on each keyword token is higher on $Android_{S}$ (i.e., 0.0125) than the $\bar{r}$ on $Android_{M}$ (i.e., 0.0052).
This result suggests that the feature importance value assigned by the SHAP approach is related to the size of the input features. 
Although there is a significant difference in the value $\bar{r}$ between different datasets, we can observe that the distribution is consistent.
For all datasets, code generation models pay the most attention to the keyword tokens (e.g., the $\bar{r}$ of keywords on $BFP{S}$ is 0.0169, which is much higher than the other four token types).
Besides that, identifiers also received high feature importance values. 
On the contrary, Figure~\ref{fig:fi4_token_types_exp_codereviewer} shows that the feature importance $\bar{r}$ of operators, separators and literals is relatively small.
These findings demonstrate that the same code generation model learns similar patterns on different datasets. 

Table~\ref{tab:tab11_code_changed_sen_Codereviewer} compares the feature importance $\bar{r}$ of changed tokens and unchanged tokens on all studied datasets for the code generation model CodeReviewer.
Interestingly, we observe a consistent relationship between the $\bar{r}$ on the changed tokens and unchanged tokens with Table~\ref{tab:tab6_exp_changes_unchanges_models} (i.e., the $\bar{r}$ of changed tokens is usually smaller than the $\bar{r}$ of unchanged tokens).
As Table~\ref{tab:tab11_code_changed_sen_Codereviewer} shows, there is a significant difference of the ratios $\bar{r}_{change}/\bar{r}_{unchange}$ on different datasets.
The ratio $\bar{r}_{change}/\bar{r}_{unchange}$ is relatively small on the datasets that have a low $CCR_{w/o}$.
For example, the ratio value is only 0.79 on the dataset $Google_{M}$ where CodeReviewer has a 62.77\% $CCR_{w/o}$, while the ratio is up to 0.94 on the dataset $java2c\#$ where CodeReviewer generates more new changed code sequences. 
These observations suggest that although the model is the same, the level to capture the changing patterns depends on the datasets. 
If the feature importance value on the changing patterns is higher, code generation models will produce more new code tokens.


\find{\textbf{Answer to RQ3:}
%SHAP is more efficient and effective in explaining code generation models.
On the same dataset, distinct code generation models capture different information to make a prediction. 
However, keywords are the most important tokens when models generate new code sequences. 
Regardless of the type of datasets, code generation models pay the most attention to keywords.
Explanation results indicate that the model pays less attention to changed tokens, resulting in lower sensitivity.
}


==> sections/threats.tex <==
\section{Threats to Validity}
\label{threats}

\textbf{Construct Validity.}
xxx

\textbf{Internal Validity.}
xxxx

\textbf{External Validity.}
xx

==> tables/tab3_sensetive_android_small.tex <==

\begin{table}[t]
  \centering
%\caption{Sensitivity of code generation models on \boldmath{}$Android_{S}$\unboldmath{} \yue{we want PL models to generate new code (i.e., AABB -> AABCD but models still do AABB -> AABB). Models are not sensitive. For T5 model, 78.9\% of inputs will get the same outputs}}
    \begin{tabular}{lrrr}
    \toprule
    \textbf{NMT models} & \multicolumn{1}{c}{\textbf{Accuray}} & \multicolumn{1}{c}{\boldmath{}\textbf{$CUR_{w}$}\unboldmath{}} & \multicolumn{1}{c}{\boldmath{}\textbf{$CUR_{w/o}$}\unboldmath{}} \\
    \midrule
    \textbf{T5} & 6.38\% & 4.87\% & 78.90\% \\
    \textbf{CodeT5} & 13.80\% & 40.37\% & 41.40\% \\
    \textbf{CoTexT} & 7.46\% & 4.51\% & 74.79\% \\
    \textbf{CodeTrans} & 7.02\% & 36.06\% & 37.42\% \\
    \textbf{CodeReviwer} & 14.72\% & 14.52\% & 15.32\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:tab3_sensetive_unchanged_android_s}%
\end{table}%




==> tables/tab4_sensetive_codereviewer.tex <==
\begin{table}[t]
  \centering
  
  \caption{Sensitivity of CodeReviewer on the studied datasets
  %\yue{Although Codereviewer has best sensitivity on Android\_{S}, but the model are not robust on other dataset. E.g., 47.23\% of inputs get no change on the dataset TOSEM'19 Medium}
  }
    \begin{tabular}{lrrr}
    \toprule
    \textbf{Datasets} & \multicolumn{1}{c}{\textbf{Accuray}} & \multicolumn{1}{c}{\boldmath{}\textbf{$CCR_{w}$}\unboldmath{}} & \multicolumn{1}{r}{\boldmath{}\textbf{$CCR_{w/o}$}\unboldmath{}} \\
    \midrule
    \boldmath{}\textbf{$Android_{S}$}\unboldmath{} & 14.72\% & 85.48\% & 84.68\% \\
    \boldmath{}\textbf{$Android_{M}$}\unboldmath{} & 10.44\% & 68.66\% & 68.07\% \\
    \boldmath{}\textbf{$Google_{S}$}\unboldmath{} & 11.81\% & 74.19\% & 73.83\% \\
    \boldmath{}\textbf{$Google_{M}$}\unboldmath{} & 6.85\% & 62.98\% & 62.77\% \\
    \boldmath{}\textbf{$Ovirt_{S}$}\unboldmath{} & 25.49\% & 89.72\% & 89.65\% \\
    \boldmath{}\textbf{$Ovirt_{M}$}\unboldmath{} & 18.18\% & 80.17\% & 79.94\% \\
    \boldmath{}\textbf{$BFP_{S}$}\unboldmath{} & 17.94\% & 89.48\% & 86.17\% \\
    \boldmath{}\textbf{$BFP_{M}$}\unboldmath{} & 8.77\% & 55.58\% & 52.77\% \\
    \boldmath{}\textbf{$FSE'22$}\unboldmath{} & 28.79\% & 85.53\% & 81.41\% \\
    \boldmath{}\textbf{$java2c\#$}\unboldmath{} & 62.10\% & 98.00\% & 97.70\% \\
    \boldmath{}\textbf{$c\#2java$}\unboldmath{} & 66.10\% & 98.30\% & 98.00\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:tab4_sensetive_unchanged_codereviewer}%
\end{table}%




==> tables/tab5_similarity_of_different_models.tex <==
\begin{table}[t]
  \centering
  \scriptsize
%\caption{Average feature importance of token types highlighted by different code generation models on $Android_{S}$. The value is $\bar{r}$ \yue{Different models have similar focus, more focus on identifiers, keywords and Separators. On top focus, we observe that models are more focus on identifier and keywords}}
    \begin{tabular}{lrrrrr}
    \toprule
    \textbf{NMT models} & \multicolumn{1}{c}{\textbf{Identifiers}} & \multicolumn{1}{c}{\textbf{Keywords}} & \multicolumn{1}{c}{\textbf{Operators}} & \multicolumn{1}{c}{\textbf{Separators}} & \multicolumn{1}{c}{\textbf{Literals}} \\
    \midrule
    \textbf{T5} & 0.0083 & 0.0126 & 0.0076 & 0.0068 & 0.0061 \\
    \textbf{CodeT5} & 0.0119 & 0.0147 & 0.0095 & 0.0101 & 0.0086 \\
    \textbf{CoTexT} & 0.0090 & 0.0142 & 0.0093 & 0.0083 & 0.0072 \\
    \textbf{CodeTrans} & 0.0114 & 0.0152 & 0.0089 & 0.0070 & 0.0102 \\
    \textbf{CodeReviwer} & 0.0113 & 0.0125 & 0.0085 & 0.0092 & 0.0085 \\
    \bottomrule
    \end{tabular}%
  \label{tab:similarity_of_token_types_of_different_models}%
\end{table}%


==> tables/tab6_exp_token_size_codereviewer.tex <==
% Table generated by Excel2LaTeX from sheet 'exp_size_tokens'
\begin{table}[t]
  \centering
  \footnotesize
%\caption{Token types of CodeReviewer \yue{Similar, but we find that when input have larger length, models are focus more on Separators, less on identifiers and keywords, -> less accurate}}
    \begin{tabular}{lrrrrr}
    \toprule
          & \multicolumn{1}{c}{\textbf{Identifiers}} & \multicolumn{1}{c}{\textbf{Keywords}} & \multicolumn{1}{c}{\textbf{Operators}} & \multicolumn{1}{c}{\textbf{Separators}} & \multicolumn{1}{c}{\textbf{Literals}} \\
    \midrule
    \boldmath{}\textbf{$Android_{S}$}\unboldmath{} & 0.0113 & 0.0125 & 0.0085 & 0.0092 & 0.0085 \\
    \boldmath{}\textbf{$Android_{M}$}\unboldmath{} & 0.0049 & 0.0052 & 0.0042 & 0.0042 & 0.0042 \\
    \boldmath{}\textbf{$Google_{S}$}\unboldmath{} & 0.0104 & 0.0123 & 0.0086 & 0.0096 & 0.0079 \\
    \boldmath{}\textbf{$Google_{M}$}\unboldmath{} & 0.0049 & 0.0055 & 0.0043 & 0.0046 & 0.0043 \\
    \boldmath{}\textbf{$Ovirt_{S}$}\unboldmath{} & 0.0090 & 0.0104 & 0.0072 & 0.0078 & 0.0075 \\
    \boldmath{}\textbf{$Ovirt_{M}$}\unboldmath{} & 0.0042 & 0.0045 & 0.0037 & 0.0038 & 0.0037 \\
    \boldmath{}\textbf{$BFP_{S}$}\unboldmath{} & 0.0109 & 0.0169 & 0.0134 & 0.0120 & 0.0131 \\
    \boldmath{}\textbf{$BFP_{M}$}\unboldmath{} & 0.0048 & 0.0073 & 0.0062 & 0.0052 & 0.0055 \\
    \boldmath{}\textbf{$java2c\#$}\unboldmath{} & 0.0126 & 0.0133 & 0.0076 & 0.0109 & 0.0068 \\
    \boldmath{}\textbf{$c\#2java$}\unboldmath{} & 0.0110 & 0.0113 & 0.0077 & 0.0105 & 0.0071 \\
    \bottomrule
    \end{tabular}%
  \label{tab:tab9_token_types_exp_codereviewer}%
\end{table}%



% % Table generated by Excel2LaTeX from sheet 'exp_size_tokens'
% \begin{table}[t]
%   \centering
%   \caption{Token Length of Codereviwer \yue{on the smaller input, models can capture more longer tokens}}
%     \begin{tabular}{lrrr}
%     \toprule
%     \textbf{Token length} & \multicolumn{1}{c}{\textbf{\textasciitilde5}} & \multicolumn{1}{c}{\textbf{5\textasciitilde10}} & \multicolumn{1}{c}{\textbf{10\textasciitilde}} \\
%     \midrule
%     \boldmath{}\textbf{$Android_{S}$}\unboldmath{} & 0.0095 & 0.0133 & 0.0106 \\
%     \boldmath{}\textbf{$Android_{M}$}\unboldmath{} & 0.0043 & 0.0056 & 0.0047 \\
%     \boldmath{}\textbf{$Google_{S}$}\unboldmath{} & 0.0095 & 0.0133 & 0.0106 \\
%     \boldmath{}\textbf{$Google_{M}$}\unboldmath{} & 0.0046 & 0.0058 & 0.0044 \\
%     \boldmath{}\textbf{$Ovirt_{S}$}\unboldmath{} & 0.0080 & 0.0112 & 0.0083 \\
%     \boldmath{}\textbf{$Ovirt_{M}$}\unboldmath{} & 0.0038 & 0.0049 & 0.0039 \\
%     \boldmath{}\textbf{$BFP_{S}$}\unboldmath{} & 0.0126 & 0.0120 & 0.0122 \\
%     \boldmath{}\textbf{$BFP_{M}$}\unboldmath{} & 0.0055 & 0.0051 & 0.0054 \\
%     \boldmath{}\textbf{$java2c\#$}\unboldmath{} & 0.0101 & 0.0144 & 0.0130 \\
%     \boldmath{}\textbf{$c\#2java$}\unboldmath{} & 0.0097 & 0.0128 & 0.0103 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:tab10_token_size_exp_codereviewer}%
% \end{table}%



==> tables/tab7_sensentive_models_explanation.tex <==
% Table generated by Excel2LaTeX from sheet 'sensetive_android_small'
\begin{table}[t]
  \centering
  \small
  \caption{Comparison of feature importance ($\bar{r}$) of changed tokens and unchanged tokens on $Android_{S}$ 
%\yue{If PL are more sensitive (more AAAB -> AABCD), explanations show that models can focus more on the updated part in the inputs}
  }
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{NMT models} & \multicolumn{1}{c}{\textbf{$CCR_{w/o}$}} & \multicolumn{1}{c}{\textbf{$\bar{r}_{change}$}} & \multicolumn{1}{c}{\textbf{$\bar{r}_{unchange}$}} & \multicolumn{1}{c}{\textbf{$\bar{r}_{change}/\bar{r}_{unchange}$}} \\
    \midrule
    \textbf{T5} & 21.10\% & 0.0092 & 0.0130 & 0.7088 \\
    \textbf{CodeT5} & 58.60\% & 0.0128 & 0.0140 & 0.9151 \\
    \textbf{CoTexT} & 25.21\% & 0.0109 & 0.0137 & 0.7981 \\
    \textbf{CodeTrans} & 62.58\% & 0.0118 & 0.0121 & 0.9756 \\
    \textbf{CodeReviwer} & 84.68\% & 0.0119 & 0.0128 & 0.9259 \\
    \bottomrule
    \end{tabular}%
  \label{tab:tab6_exp_changes_unchanges_models}%
\end{table}%


==> tables/tab8_explanation_compare.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet2'
\begin{table}[t]
  \centering
  \small
  \caption{Comparison with different XAI techniques 
%\yue{Updating. but the results have been observed. SHAP is more efficient than Sailiency and IG (less time, less resource usage). SHAP is more accurate than Attention (better capture model behaviors, bigger range, and standard variance )}
  }
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{Approach} & \multicolumn{1}{c}{\textbf{Memory (MB)}} & \multicolumn{1}{c}{\textbf{Time (s)}} & \multicolumn{1}{c}{\boldmath{}\textbf{Range ($\bar{r}$)}\unboldmath{}} & \multicolumn{1}{c}{\boldmath{}\textbf{StdDev($\bar{r}$)}\unboldmath{}} \\
    \midrule
    \textbf{Attention } & 3029  & 0.47  & 4.12E-03 & 1.02E-03 \\
    \textbf{IG} & 16864 & 5.62  & 1.74E-02 & 4.81E-03 \\
    \textbf{SHAP} & 3842  & 2.34  & 1.23E-02 & 3.16E-03 \\
    \bottomrule
    \end{tabular}%
  \label{tab:tab_compare_exp_methods}%
\end{table}%


==> tables/tab9_sensetive_diffrent_data_codereviewer_exp.tex <==
% Table generated by Excel2LaTeX from sheet 'sensetive_code_reviewer'
\begin{table}[t]
  \centering
  \footnotesize
  \caption{Comparison of feature importance ($\bar{r}$) of changed tokens and unchanged tokens generated by CodeReviewer on the studied datasets 
    %\yue{On different dataset, if model are sensitive on the dataset, models usually focus more on changed tokens}
  }
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{Datasets}  & \multicolumn{1}{c}{\textbf{$CCR_{w/o}$}} & \multicolumn{1}{c}{\textbf{$\bar{r}_{change}$}} & \multicolumn{1}{c}{\textbf{$\bar{r}_{unchange}$}} & \multicolumn{1}{c}{\textbf{$\bar{r}_{change}/\bar{r}_{unchange}$}}  \\
    \midrule
    \boldmath{}\textbf{$Android_{S}$}\unboldmath{} & 84.68\% & 0.0119 & 0.0128 & 0.9259 \\
    \boldmath{}\textbf{$Android_{M}$}\unboldmath{} & 68.07\% & 0.0044 & 0.0055 & 0.7920 \\
    \boldmath{}\textbf{$Google_{S}$}\unboldmath{} & 73.83\% & 0.0115 & 0.0127 & 0.9038 \\
    \boldmath{}\textbf{$Google_{M}$}\unboldmath{} & 62.77\% & 0.0046 & 0.0058 & 0.7941 \\
    \boldmath{}\textbf{$Ovirt_{S}$}\unboldmath{} & 89.65\% & 0.0098 & 0.0101 & 0.9656 \\
    \boldmath{}\textbf{$Ovirt_{M}$}\unboldmath{} & 79.94\% & 0.0039 & 0.0048 & 0.8022 \\
    \boldmath{}\textbf{$BFP_{S}$}\unboldmath{} & 86.17\% & 0.0121 & 0.0145 & 0.8345 \\
    \boldmath{}\textbf{$BFP_{M}$}\unboldmath{} & 52.77\% & 0.0047 & 0.0057 & 0.8131 \\
    \boldmath{}\textbf{$FSE'22$}\unboldmath{} & 81.41\% & 0.0064 & 0.0076 & 0.8520 \\
    \boldmath{}\textbf{$java2c\#$}\unboldmath{} & 97.70\% & 0.0210 & 0.0205 & 0.9381 \\
    \boldmath{}\textbf{$c\#2java$}\unboldmath{} & 98.00\% & 0.0158 & 0.0172 & 0.9185 \\
    \bottomrule
    \end{tabular}%
  \label{tab:tab11_code_changed_sen_Codereviewer}%
\end{table}%



